Deep Structural Causal Models for Tractable Counterfactual Inference

We formulate a general framework for building structural causal models (SCMs) with deep learning components. The proposed approach employs normalising flows and variational inference to enable tractable inference of exogenous noise variables - a crucial step for counterfactual inference that is missing from existing deep causal learning methods. Our framework is validated on a synthetic dataset built on MNIST as well as on a real-world medical dataset of brain MRI scans. Our experimental results indicate that we can successfully train deep SCMs that are capable of all three levels of Pearl's ladder of causation: association, intervention, and counterfactuals, giving rise to a powerful new approach for answering causal questions in imaging applications and beyond. The code for all our experiments is available at https://github.com/biomedia-mira/deepscm.

==> figures/mechanisms/ael.tex <==
\begin{subfigure}[b]{.3\textwidth}
\centering
% \begin{tikzpicture}
%   \node[latent]                         (exhi) {$\noisehi_k$};
%   \node[latent, below=of exhi]            (exlo) {$\noiselo_k$};
%   \node[obs, left=of exlo]          (x) {$x_k$};
%   \node[const, outer sep=2pt, left=of exhi] (pa) {$\pak$};
%   \node[aux] at ($(x)+(.5,.5)$) (h) {};
%   \node[aux, below=0.5 of pa] (k) {};

%   \edge[-]{pa, exhi}{h};
%   \edge[-, amort]{pa, x}{k};
%   \draw[-{Latex[open]}, amort] (k) edge[bend left=15] node[pos=.6, above] {$\encoder_k$} (exhi);

%   \draw[invertible] (exlo) -- (x) node[midway, below] {$\mechlo_k$} coordinate[midway] (fx);
%   \draw[-Circle] (h) -- (fx) node[near start, right] {$\mechhi_k$};
% \end{tikzpicture}
\begin{tikzpicture}
  \node[latent] at (.5,.8)                         (exhi) {$\noisehi_k$};
  \node[latent] at (1,0)            (exlo) {$\noiselo_k$};
  \node[obs] at (0,0)          (x) {$x_k$};
  \node[const, outer sep=2pt] at (-.5,.8) (pa) {$\pak$};
  \node[aux] at ($(x)+(.5,.4)$) (h) {};
%   \node[aux, below=0.5 of pa] (k) {};

  \draw[-{Latex[open]}, amort] (x) edge[bend left]
    node[midway, aux] (k) {}
    node[pos=.75, above left=-3pt] {$\encoder_k$}
    (exhi);
  \edge[-]{exhi}{h};
  \draw[-] (pa) edge[bend right] (h);
  \edge[-, amort]{pa}{k};
%   \draw[-{Latex[open]}, amort] (k) edge[bend left=15] node[pos=.6, above] {$\encoder_k$} (exhi);

  \draw[invertible] (exlo) -- (x) node[midway, below] {$\mechlo_k$} coordinate[midway] (fx);
  \draw[-Circle] (h) -- (fx) node[near start, right] {$\mechhi_k$};
\end{tikzpicture}
%\caption{Hybrid mechanism}
\caption{Amortised explicit likelihood}
\label{fig:mech_ae}
\end{subfigure}

==> figures/mechanisms/ail.tex <==
\begin{subfigure}[b]{.3\textwidth}
\centering
% \begin{tikzpicture}
%   \node[latent] at (1,1)                 (exhi) {$\noise_k$};
%   \node[obs] at (1,0)          (x) {$x_k$};
%   \node[const, outer sep=2pt] at (.13,.5) (pa) {$\pak$};

%   \draw[->] (exhi) edge[bend left]
%     node[midway, aux] (h) {}
%     node[pos=.75, right] {$\mech_k$}
%     (x);
%   \draw[-{Latex[open]}, amort] (x) edge[bend left]
%     node[midway, aux] (k) {}
%     node[pos=.75, above left] {$\encoder_k$}
%     (exhi);
%   \draw[-] (pa) edge[bend left=20] (h);
%   \draw[-, amort] (pa) edge[bend right=20] (k);
% \end{tikzpicture}
\begin{tikzpicture}
  \node[latent] at (1,1)                 (exhi) {$\noise_k$};
  \node[obs] at (1,0)          (x) {$x_k$};
  \node[const, outer sep=2pt] at (.3,1) (pa) {$\pak$};

  \draw[->] (exhi) edge[bend right]
    node[midway, aux] (h) {}
    node[pos=.75, left] {$\mech_k$}
    (x);
  \draw[-{Latex[open]}, amort] (x) edge[bend right]
    node[midway, aux] (k) {}
    node[pos=.75, right] {$\encoder_k$}
    (exhi);
  \draw[-] (pa) edge (h);
  \draw[-, amort] (pa) edge (k);
\end{tikzpicture}
%\caption{\wip{Autoencoding/implicit mechanism}}
\caption{Amortised implicit likelihood}
\label{fig:mech_ai}
\end{subfigure}%

==> figures/mechanisms/iel.tex <==
\begin{subfigure}[b]{.3\textwidth}
\centering
\begin{tikzpicture}
  \node[latent] at (1,0)            (exlo) {$\noise_k$};
  \node[obs] at (0,0)          (x) {$x_k$};
  \node[const, outer sep=2pt] at (.5,.87) (pa) {$\pak$};

  \draw[invertible] (exlo) -- (x) node[midway, below] {$\mech_k$} coordinate[midway] (fx);
  \draw[-Circle] (pa) -- (fx);
\end{tikzpicture}
%\caption{Invertible mechanism}
\caption{Invertible explicit likelihood}
\label{fig:mech_ie}
\end{subfigure}%

==> figures/medical/graphical_models/causal_graph_medical.tex <==
\begin{tikzpicture}[x=12mm, y=10mm]
  \node[cvar, label={left:age}]                  (a) {};
  \node[cvar, label={right:sex}, right=1 of a]                  (s) {};
  \node[cvar, label={[align=right]left:ventricle\\volume}, below=1 of a]                  (v) {};
  \node[cvar, label={[align=left]right:brain\\volume}, below=1 of s]                  (b) {};
  \node[cvar, label={right:image}] at ($(v)+(.5,-.87)$)                  (x) {};
  
  \edge{a, s}{b}
  \edge{a, b}{v}
  \edge{b, v}{x}
\end{tikzpicture}

==> figures/medical/graphical_models/covariate_sem.tex <==
\begin{tikzpicture}

  % Define nodes
  \node[latent]                            (ea) {$\noise_{age}$};
  \node[det, below=of ea]                  (a) {$age$};
  
  \node[latent, right=of ea]               (es) {$\noise_{sex}$};
  \node[det, below=of es]                  (s) {$sex$};
  
  \node[latent, left= of a]               (ev) {$\noise_{v}$};
  \node[det, below=of a]                  (v) {$v$};
  
  \node[latent, right=of s]               (eb) {$\noise_{b}$};
  \node[det, below=of s]                  (b) {$b$};
  
  \node[latent, right=of b]               (ex) {$\noise_{x}$};
  \node[det, below=of ex]                  (x) {$x$};
  
  \edge{et}{t}
  \edge{es}{s}
  \edge{eb, a, s}{b}
  \edge{ev, a, b}{v}
  \edge{ex, b, v}{x}
\end{tikzpicture}
\begin{tikzpicture}[x=12mm, y=10mm]
  \node[cvar, label={left:age}]                  (a) {};
  \node[cvar, label={right:sex}, right=1 of a]                  (s) {};
  \node[cvar, label={[align=right]left:ventricle\\volume}, below=1 of a]                  (v) {};
  \node[cvar, label={[align=left]right:brain\\volume}, below=1 of s]                  (b) {};
  \node[cvar, label={right:image}] at ($(v)+(.5,-.87)$)                  (x) {};
  
  \edge{a, s}{b}
  \edge{a, b}{v}
  \edge{b, v}{x}
\end{tikzpicture}

==> figures/morphomnist/graphical_models/sem_abduction.tex <==
\begin{tikzpicture}
  % Define nodes
  \node[det]                            (et) {$\noise_T$};
  \node[obs, below=of et]                  (t) {$t$};
  
  \node[det, right=of et]               (ei) {$\noise_I$};
  \node[obs, below=of ei]                  (i) {$i$};
  
  \node[latent, right=of i]               (exhi) {$\noisehi_X$};
  \node[det, below=of exhi]            (exlo) {$\noiselo_X$};
  \node[obs, left=of exlo]                  (x) {$x$};
  
  \edge{t}{et}
  \edge{i, t}{ei}
  \edge[amort]{x, i}{exhi}
  \draw[->, amort] (t) edge[bend right] (exhi);
  \edge{x, exhi, t, i}{exlo}
\end{tikzpicture}
